Do Cookie Banners Respect my Choice? Measuring Legal Compliance of Banners from IAB Europe's Transparency and Consent Framework

As a result of the GDPR and the ePrivacy Directive, European users encounter cookie banners on almost every website. Many of such banners are implemented by Consent Management Providers (CMPs), who respect the IAB Europe's Transparency and Consent Framework (TCF). Via cookie banners, CMPs collect and disseminate user consent to third parties. In this work, we systematically study IAB Europe's TCF and analyze consent stored behind the user interface of TCF cookie banners. We analyze the GDPR and the ePrivacy Directive to identify legal violations in implementations of cookie banners based on the storage of consent and detect such violations by crawling 22 949 European websites. With two automatic and semi-automatic crawl campaigns, we detect violations, and we find that: 141 websites register positive consent even if the user has not made their choice; 236 websites nudge the users towards accepting consent by pre-selecting options; and 27 websites store a positive consent even if the user has explicitly opted out. Performing extensive tests on 560 websites, we find at least one violation in 54% of them. Finally, we provide a browser extension to facilitate manual detection of violations for regular users and Data Protection Authorities.

==> tables/cmp_table_gdpr_nonrespect.tex <==
                           Evidon & \cellcolor{BrickRed!25} 25.0\% (4/16) & \cellcolor{BrickRed!22} 22.2\% (2/9) &                    -  &                    -  &                    -  &                    -  & \cellcolor{BrickRed!28} 28.6\% (2/7)\\
                         OneTrust & \cellcolor{BrickRed!8} 8.3\% (4/48) & \cellcolor{BrickRed!6} 6.7\% (1/15) & \cellcolor{BrickRed!0} 0.0\% (0/6) & \cellcolor{BrickRed!0} 0.0\% (0/4) & \cellcolor{BrickRed!11} 11.1\% (1/9) & \cellcolor{BrickRed!0} 0.0\% (0/3) & \cellcolor{BrickRed!18} 18.2\% (2/11)\\
                          WEBEDIA & \cellcolor{BrickRed!100} 100.0\% (3/3) &                    -  & \cellcolor{BrickRed!100} 100.0\% (3/3) &                    -  &                    -  &                    -  &                    - \\
                  Livesport Media & \cellcolor{BrickRed!100} 100.0\% (3/3) &                    -  & \cellcolor{BrickRed!100} 100.0\% (1/1) & \cellcolor{BrickRed!100} 100.0\% (1/1) &                    -  &                    -  & \cellcolor{BrickRed!100} 100.0\% (1/1)\\
                           M6 Web & \cellcolor{BrickRed!75} 75.0\% (3/4) &                    -  & \cellcolor{BrickRed!75} 75.0\% (3/4) &                    -  &                    -  &                    -  &                    - \\
                  \textbf{others} & \cellcolor{BrickRed!2} 2.3\% (10/434) & \cellcolor{BrickRed!0} 0.0\% (0/119) & \cellcolor{BrickRed!2} 2.5\% (3/119) & \cellcolor{BrickRed!1} 2.0\% (2/101) & \cellcolor{BrickRed!0} 0.0\% (0/13) & \cellcolor{BrickRed!0} 0.0\% (0/16) & \cellcolor{BrickRed!7} 7.6\% (5/66)\\
\hline
           \setrow{\bfseries} all & \cellcolor{BrickRed!5} 5.3\% (27/508) & \cellcolor{BrickRed!2} 2.1\% (3/143) & \cellcolor{BrickRed!7} 7.5\% (10/133) & \cellcolor{BrickRed!2} 2.8\% (3/106) & \cellcolor{BrickRed!4} 4.5\% (1/22) & \cellcolor{BrickRed!0} 0.0\% (0/19) & \cellcolor{BrickRed!11} 11.8\% (10/85)\\
\hline


==> tables/cmp_table_gdpr_nooption.tex <==
                        Quantcast & \cellcolor{BrickRed!5} 5.2\% (9/174) & \cellcolor{BrickRed!0} 0.0\% (0/60) & \cellcolor{BrickRed!0} 0.0\% (0/34) & \cellcolor{BrickRed!23} 23.1\% (9/39) & \cellcolor{BrickRed!0} 0.0\% (0/5) & \cellcolor{BrickRed!0} 0.0\% (0/12) & \cellcolor{BrickRed!0} 0.0\% (0/24)\\
                    Axel Springer & \cellcolor{BrickRed!70} 70.0\% (7/10) &                    -  & \cellcolor{BrickRed!100} 100.0\% (1/1) & \cellcolor{BrickRed!83} 83.3\% (5/6) &                    -  &                    -  & \cellcolor{BrickRed!33} 33.3\% (1/3)\\
                           Evidon & \cellcolor{BrickRed!22} 22.7\% (5/22) & \cellcolor{BrickRed!10} 10.0\% (1/10) & \cellcolor{BrickRed!100} 100.0\% (1/1) &                    -  & \cellcolor{BrickRed!100} 100.0\% (1/1) & \cellcolor{BrickRed!50} 50.0\% (1/2) & \cellcolor{BrickRed!12} 12.5\% (1/8)\\
            Global Radio Services & \cellcolor{BrickRed!100} 100.0\% (3/3) & \cellcolor{BrickRed!100} 100.0\% (3/3) &                    -  &                    -  &                    -  &                    -  &                    - \\
                  \textbf{others} & \cellcolor{BrickRed!3} 4.0\% (14/351) & \cellcolor{BrickRed!2} 2.6\% (2/76) & \cellcolor{BrickRed!2} 2.9\% (3/103) & \cellcolor{BrickRed!2} 2.6\% (2/78) & \cellcolor{BrickRed!9} 9.5\% (2/21) & \cellcolor{BrickRed!9} 9.1\% (1/11) & \cellcolor{BrickRed!6} 6.5\% (4/62)\\
\hline
           \setrow{\bfseries} all & \cellcolor{BrickRed!6} 6.8\% (38/560) & \cellcolor{BrickRed!4} 4.0\% (6/149) & \cellcolor{BrickRed!3} 3.6\% (5/139) & \cellcolor{BrickRed!13} 13.0\% (16/123) & \cellcolor{BrickRed!11} 11.1\% (3/27) & \cellcolor{BrickRed!8} 8.0\% (2/25) & \cellcolor{BrickRed!6} 6.2\% (6/97)\\
\hline


==> tables/cmp_table_gdpr_per_country.tex <==
&\multicolumn{6}{l}{\bf Non-respect of decision} \\ \hline
                Conversant Europe & \cellcolor{BrickRed!100} 100.00 \% (   4/   4) & \cellcolor{BrickRed!100} 100.00 \% (   1/   1) &                    -  & \cellcolor{BrickRed!100} 100.00 \% (   3/   3) &                    -  &                    - \\\hline
                   Commanders Act & \cellcolor{BrickRed!27}  27.27 \% (   3/  11) &                    -  & \cellcolor{BrickRed!27}  27.27 \% (   3/  11) &                    -  &                    -  &                    - \\\hline
                           M6 Web & \cellcolor{BrickRed!75}  75.00 \% (   3/   4) &                    -  & \cellcolor{BrickRed!75}  75.00 \% (   3/   4) &                    -  &                    -  &                    - \\\hline
                           Evidon & \cellcolor{BrickRed!14}  14.29 \% (   2/  14) & \cellcolor{BrickRed!20}  20.00 \% (   2/  10) & \cellcolor{BrickRed!0}   0.00 \% (   0/   1) &                    -  & \cellcolor{BrickRed!0}   0.00 \% (   0/   1) & \cellcolor{BrickRed!0}   0.00 \% (   0/   2)\\\hline
                          WEBEDIA & \cellcolor{BrickRed!75}  75.00 \% (   3/   4) &                    -  & \cellcolor{BrickRed!75}  75.00 \% (   3/   4) &                    -  &                    -  &                    - \\\hline
              Snigel Web Services & \cellcolor{BrickRed!100} 100.00 \% (   2/   2) &                    -  & \cellcolor{BrickRed!100} 100.00 \% (   1/   1) &                    -  &                    -  & \cellcolor{BrickRed!100} 100.00 \% (   1/   1)\\\hline
                         OneTrust & \cellcolor{BrickRed!5}   5.26 \% (   2/  38) & \cellcolor{BrickRed!6}   6.25 \% (   1/  16) & \cellcolor{BrickRed!0}   0.00 \% (   0/   6) & \cellcolor{BrickRed!0}   0.00 \% (   0/   4) & \cellcolor{BrickRed!11}  11.11 \% (   1/   9) & \cellcolor{BrickRed!0}   0.00 \% (   0/   3)\\\hline
                 Groupe Sud Ouest & \cellcolor{BrickRed!100} 100.00 \% (   2/   2) &                    -  & \cellcolor{BrickRed!100} 100.00 \% (   2/   2) &                    -  &                    -  &                    - \\\hline
                  Livesport Media & \cellcolor{BrickRed!100} 100.00 \% (   2/   2) &                    -  & \cellcolor{BrickRed!100} 100.00 \% (   1/   1) & \cellcolor{BrickRed!100} 100.00 \% (   1/   1) &                    -  &                    - \\\hline
                            Publy & \cellcolor{BrickRed!100} 100.00 \% (   2/   2) &                    -  &                    -  & \cellcolor{BrickRed!100} 100.00 \% (   2/   2) &                    -  &                    - \\\hline
                  \textbf{others} & \cellcolor{BrickRed!0}   0.81 \% (   3/ 371) & \cellcolor{BrickRed!0}   0.00 \% (   0/ 113) & \cellcolor{BrickRed!0}   0.92 \% (   1/ 109) & \cellcolor{BrickRed!1}   1.77 \% (   2/ 113) & \cellcolor{BrickRed!0}   0.00 \% (   0/  17) & \cellcolor{BrickRed!0}   0.00 \% (   0/  19)\\\hline
                     \textbf{all} & \cellcolor{BrickRed!6}   6.17 \% (  28/ 454) & \cellcolor{BrickRed!2}   2.86 \% (   4/ 140) & \cellcolor{BrickRed!10}  10.07 \% (  14/ 139) & \cellcolor{BrickRed!6}   6.50 \% (   8/ 123) & \cellcolor{BrickRed!3}   3.70 \% (   1/  27) & \cellcolor{BrickRed!4}   4.00 \% (   1/  25)\\\hline
&\multicolumn{6}{l}{\bf No option} \\ \hline
                        Quantcast & \cellcolor{BrickRed!6}   6.21 \% (   9/ 145) & \cellcolor{BrickRed!0}   0.00 \% (   0/  59) & \cellcolor{BrickRed!0}   0.00 \% (   0/  34) & \cellcolor{BrickRed!25}  25.00 \% (   9/  36) & \cellcolor{BrickRed!0}   0.00 \% (   0/   5) & \cellcolor{BrickRed!0}   0.00 \% (   0/  11)\\\hline
                    Axel Springer & \cellcolor{BrickRed!85}  85.71 \% (   6/   7) &                    -  & \cellcolor{BrickRed!100} 100.00 \% (   1/   1) & \cellcolor{BrickRed!83}  83.33 \% (   5/   6) &                    -  &                    - \\\hline
                           Evidon & \cellcolor{BrickRed!28}  28.57 \% (   4/  14) & \cellcolor{BrickRed!10}  10.00 \% (   1/  10) & \cellcolor{BrickRed!100} 100.00 \% (   1/   1) &                    -  & \cellcolor{BrickRed!100} 100.00 \% (   1/   1) & \cellcolor{BrickRed!50}  50.00 \% (   1/   2)\\\hline
            Global Radio Services & \cellcolor{BrickRed!100} 100.00 \% (   3/   3) & \cellcolor{BrickRed!100} 100.00 \% (   3/   3) &                    -  &                    -  &                    -  &                    - \\\hline
                 Cookie Trust WG. & \cellcolor{BrickRed!25}  25.00 \% (   2/   8) &                    -  & \cellcolor{BrickRed!33}  33.33 \% (   1/   3) & \cellcolor{BrickRed!33}  33.33 \% (   1/   3) & \cellcolor{BrickRed!0}   0.00 \% (   0/   2) &                    - \\\hline
                  \textbf{others} & \cellcolor{BrickRed!2}   2.89 \% (   8/ 277) & \cellcolor{BrickRed!2}   2.94 \% (   2/  68) & \cellcolor{BrickRed!2}   2.00 \% (   2/ 100) & \cellcolor{BrickRed!1}   1.28 \% (   1/  78) & \cellcolor{BrickRed!10}  10.53 \% (   2/  19) & \cellcolor{BrickRed!8}   8.33 \% (   1/  12)\\\hline
                     \textbf{all} & \cellcolor{BrickRed!7}   7.05 \% (  32/ 454) & \cellcolor{BrickRed!4}   4.29 \% (   6/ 140) & \cellcolor{BrickRed!3}   3.60 \% (   5/ 139) & \cellcolor{BrickRed!13}  13.01 \% (  16/ 123) & \cellcolor{BrickRed!11}  11.11 \% (   3/  27) & \cellcolor{BrickRed!8}   8.00 \% (   2/  25)\\\hline
&\multicolumn{6}{l}{\bf Pre-action consent} \\ \hline
                         OneTrust & \cellcolor{BrickRed!78}  78.95 \% (  30/  38) & \cellcolor{BrickRed!81}  81.25 \% (  13/  16) & \cellcolor{BrickRed!66}  66.67 \% (   4/   6) & \cellcolor{BrickRed!25}  25.00 \% (   1/   4) & \cellcolor{BrickRed!100} 100.00 \% (   9/   9) & \cellcolor{BrickRed!100} 100.00 \% (   3/   3)\\\hline
                        Quantcast & \cellcolor{BrickRed!4}   4.14 \% (   6/ 145) & \cellcolor{BrickRed!0}   0.00 \% (   0/  59) & \cellcolor{BrickRed!0}   0.00 \% (   0/  34) & \cellcolor{BrickRed!13}  13.89 \% (   5/  36) & \cellcolor{BrickRed!20}  20.00 \% (   1/   5) & \cellcolor{BrickRed!0}   0.00 \% (   0/  11)\\\hline
                    Axel Springer & \cellcolor{BrickRed!71}  71.43 \% (   5/   7) &                    -  & \cellcolor{BrickRed!0}   0.00 \% (   0/   1) & \cellcolor{BrickRed!83}  83.33 \% (   5/   6) &                    -  &                    - \\\hline
                   Commanders Act & \cellcolor{BrickRed!36}  36.36 \% (   4/  11) &                    -  & \cellcolor{BrickRed!36}  36.36 \% (   4/  11) &                    -  &                    -  &                    - \\\hline
            Global Radio Services & \cellcolor{BrickRed!100} 100.00 \% (   3/   3) & \cellcolor{BrickRed!100} 100.00 \% (   3/   3) &                    -  &                    -  &                    -  &                    - \\\hline
                 Cookie Trust WG. & \cellcolor{BrickRed!25}  25.00 \% (   2/   8) &                    -  & \cellcolor{BrickRed!0}   0.00 \% (   0/   3) & \cellcolor{BrickRed!0}   0.00 \% (   0/   3) & \cellcolor{BrickRed!100} 100.00 \% (   2/   2) &                    - \\\hline
                  Livesport Media & \cellcolor{BrickRed!100} 100.00 \% (   2/   2) &                    -  & \cellcolor{BrickRed!100} 100.00 \% (   1/   1) & \cellcolor{BrickRed!100} 100.00 \% (   1/   1) &                    -  &                    - \\\hline
                  \textbf{others} & \cellcolor{BrickRed!1}   1.25 \% (   3/ 240) & \cellcolor{BrickRed!1}   1.61 \% (   1/  62) & \cellcolor{BrickRed!1}   1.20 \% (   1/  83) & \cellcolor{BrickRed!0}   0.00 \% (   0/  73) & \cellcolor{BrickRed!0}   0.00 \% (   0/  11) & \cellcolor{BrickRed!9}   9.09 \% (   1/  11)\\\hline
                     \textbf{all} & \cellcolor{BrickRed!12}  12.11 \% (  55/ 454) & \cellcolor{BrickRed!12}  12.14 \% (  17/ 140) & \cellcolor{BrickRed!7}   7.19 \% (  10/ 139) & \cellcolor{BrickRed!9}   9.76 \% (  12/ 123) & \cellcolor{BrickRed!44}  44.44 \% (  12/  27) & \cellcolor{BrickRed!16}  16.00 \% (   4/  25)\\\hline
&\multicolumn{6}{l}{\bf Pre-ticked} \\ \hline
                        Quantcast & \cellcolor{BrickRed!37}  37.93 \% (  55/ 145) & \cellcolor{BrickRed!55}  55.93 \% (  33/  59) & \cellcolor{BrickRed!32}  32.35 \% (  11/  34) & \cellcolor{BrickRed!11}  11.11 \% (   4/  36) & \cellcolor{BrickRed!60}  60.00 \% (   3/   5) & \cellcolor{BrickRed!36}  36.36 \% (   4/  11)\\\hline
                         OneTrust & \cellcolor{BrickRed!84}  84.21 \% (  32/  38) & \cellcolor{BrickRed!87}  87.50 \% (  14/  16) & \cellcolor{BrickRed!83}  83.33 \% (   5/   6) & \cellcolor{BrickRed!100} 100.00 \% (   4/   4) & \cellcolor{BrickRed!77}  77.78 \% (   7/   9) & \cellcolor{BrickRed!66}  66.67 \% (   2/   3)\\\hline
                      Sourcepoint & \cellcolor{BrickRed!72}  72.41 \% (  21/  29) & \cellcolor{BrickRed!100} 100.00 \% (  21/  21) & \cellcolor{BrickRed!0}   0.00 \% (   0/   8) &                    -  &                    -  &                    - \\\hline
                           Didomi & \cellcolor{BrickRed!38}  38.89 \% (  14/  36) & \cellcolor{BrickRed!100} 100.00 \% (   1/   1) & \cellcolor{BrickRed!25}  25.00 \% (   7/  28) & \cellcolor{BrickRed!0}   0.00 \% (   0/   1) & \cellcolor{BrickRed!100} 100.00 \% (   6/   6) &                    - \\\hline
                   Commanders Act & \cellcolor{BrickRed!81}  81.82 \% (   9/  11) &                    -  & \cellcolor{BrickRed!81}  81.82 \% (   9/  11) &                    -  &                    -  &                    - \\\hline
                  Improve Digital & \cellcolor{BrickRed!80}  80.00 \% (   8/  10) &                    -  & \cellcolor{BrickRed!100} 100.00 \% (   1/   1) & \cellcolor{BrickRed!77}  77.78 \% (   7/   9) &                    -  &                    - \\\hline
                        Ensighten & \cellcolor{BrickRed!100} 100.00 \% (   7/   7) & \cellcolor{BrickRed!100} 100.00 \% (   7/   7) &                    -  &                    -  &                    -  &                    - \\\hline
                Conversant Europe & \cellcolor{BrickRed!100} 100.00 \% (   4/   4) & \cellcolor{BrickRed!100} 100.00 \% (   1/   1) &                    -  & \cellcolor{BrickRed!100} 100.00 \% (   3/   3) &                    -  &                    - \\\hline
                              SFR & \cellcolor{BrickRed!100} 100.00 \% (   4/   4) &                    -  & \cellcolor{BrickRed!100} 100.00 \% (   4/   4) &                    -  &                    -  &                    - \\\hline
                 Cookie Trust WG. & \cellcolor{BrickRed!37}  37.50 \% (   3/   8) &                    -  & \cellcolor{BrickRed!66}  66.67 \% (   2/   3) & \cellcolor{BrickRed!33}  33.33 \% (   1/   3) & \cellcolor{BrickRed!0}   0.00 \% (   0/   2) &                    - \\\hline
                       Spil Games & \cellcolor{BrickRed!100} 100.00 \% (   3/   3) & \cellcolor{BrickRed!100} 100.00 \% (   1/   1) & \cellcolor{BrickRed!100} 100.00 \% (   1/   1) & \cellcolor{BrickRed!100} 100.00 \% (   1/   1) &                    -  &                    - \\\hline
                           OneTag & \cellcolor{BrickRed!100} 100.00 \% (   3/   3) &                    -  &                    -  & \cellcolor{BrickRed!100} 100.00 \% (   3/   3) &                    -  &                    - \\\hline
                             Oath & \cellcolor{BrickRed!25}  25.00 \% (   2/   8) & \cellcolor{BrickRed!0}   0.00 \% (   0/   5) & \cellcolor{BrickRed!66}  66.67 \% (   2/   3) &                    -  &                    -  &                    - \\\hline
                          WEBEDIA & \cellcolor{BrickRed!50}  50.00 \% (   2/   4) &                    -  & \cellcolor{BrickRed!50}  50.00 \% (   2/   4) &                    -  &                    -  &                    - \\\hline
                        Cookiebot & \cellcolor{BrickRed!66}  66.67 \% (   2/   3) & \cellcolor{BrickRed!100} 100.00 \% (   1/   1) & \cellcolor{BrickRed!0}   0.00 \% (   0/   1) & \cellcolor{BrickRed!100} 100.00 \% (   1/   1) &                    -  &                    - \\\hline
                           M6 Web & \cellcolor{BrickRed!50}  50.00 \% (   2/   4) &                    -  & \cellcolor{BrickRed!50}  50.00 \% (   2/   4) &                    -  &                    -  &                    - \\\hline
                  Livesport Media & \cellcolor{BrickRed!100} 100.00 \% (   2/   2) &                    -  & \cellcolor{BrickRed!100} 100.00 \% (   1/   1) & \cellcolor{BrickRed!100} 100.00 \% (   1/   1) &                    -  &                    - \\\hline
                            Publy & \cellcolor{BrickRed!100} 100.00 \% (   2/   2) &                    -  &                    -  & \cellcolor{BrickRed!100} 100.00 \% (   2/   2) &                    -  &                    - \\\hline
                  \textbf{others} & \cellcolor{BrickRed!10}  10.94 \% (  14/ 128) & \cellcolor{BrickRed!14}  14.29 \% (   4/  28) & \cellcolor{BrickRed!19}  19.23 \% (   5/  26) & \cellcolor{BrickRed!5}   5.08 \% (   3/  59) & \cellcolor{BrickRed!20}  20.00 \% (   1/   5) & \cellcolor{BrickRed!10}  10.00 \% (   1/  10)\\\hline
                     \textbf{all} & \cellcolor{BrickRed!42}  42.51 \% ( 193/ 454) & \cellcolor{BrickRed!59}  59.29 \% (  83/ 140) & \cellcolor{BrickRed!40}  40.29 \% (  56/ 139) & \cellcolor{BrickRed!24}  24.39 \% (  30/ 123) & \cellcolor{BrickRed!62}  62.96 \% (  17/  27) & \cellcolor{BrickRed!28}  28.00 \% (   7/  25)\\\hline


==> tables/cmp_table_gdpr_preaction.tex <==
                         OneTrust & \cellcolor{BrickRed!74} 74.0\% (37/50) & \cellcolor{BrickRed!81} 81.2\% (13/16) & \cellcolor{BrickRed!66} 66.7\% (4/6) & \cellcolor{BrickRed!25} 25.0\% (1/4) & \cellcolor{BrickRed!100} 100.0\% (9/9) & \cellcolor{BrickRed!100} 100.0\% (3/3) & \cellcolor{BrickRed!58} 58.3\% (7/12)\\
                    Axel Springer & \cellcolor{BrickRed!60} 60.0\% (6/10) &                    -  & \cellcolor{BrickRed!0} 0.0\% (0/1) & \cellcolor{BrickRed!83} 83.3\% (5/6) &                    -  &                    -  & \cellcolor{BrickRed!33} 33.3\% (1/3)\\
                        Quantcast & \cellcolor{BrickRed!3} 3.4\% (6/174) & \cellcolor{BrickRed!0} 0.0\% (0/60) & \cellcolor{BrickRed!0} 0.0\% (0/34) & \cellcolor{BrickRed!12} 12.8\% (5/39) & \cellcolor{BrickRed!20} 20.0\% (1/5) & \cellcolor{BrickRed!0} 0.0\% (0/12) & \cellcolor{BrickRed!0} 0.0\% (0/24)\\
                   Commanders Act & \cellcolor{BrickRed!40} 40.0\% (4/10) &                    -  & \cellcolor{BrickRed!40} 40.0\% (4/10) &                    -  &                    -  &                    -  &                    - \\
            Global Radio Services & \cellcolor{BrickRed!100} 100.0\% (3/3) & \cellcolor{BrickRed!100} 100.0\% (3/3) &                    -  &                    -  &                    -  &                    -  &                    - \\
                  Livesport Media & \cellcolor{BrickRed!100} 100.0\% (3/3) &                    -  & \cellcolor{BrickRed!100} 100.0\% (1/1) & \cellcolor{BrickRed!100} 100.0\% (1/1) &                    -  &                    -  & \cellcolor{BrickRed!100} 100.0\% (1/1)\\
                  \textbf{others} & \cellcolor{BrickRed!1} 1.9\% (6/310) & \cellcolor{BrickRed!1} 1.4\% (1/70) & \cellcolor{BrickRed!1} 1.1\% (1/87) & \cellcolor{BrickRed!0} 0.0\% (0/73) & \cellcolor{BrickRed!15} 15.4\% (2/13) & \cellcolor{BrickRed!0} 0.0\% (0/10) & \cellcolor{BrickRed!3} 3.5\% (2/57)\\
\hline
           \setrow{\bfseries} all & \cellcolor{BrickRed!11} 11.6\% (65/560) & \cellcolor{BrickRed!11} 11.4\% (17/149) & \cellcolor{BrickRed!7} 7.2\% (10/139) & \cellcolor{BrickRed!9} 9.8\% (12/123) & \cellcolor{BrickRed!44} 44.4\% (12/27) & \cellcolor{BrickRed!12} 12.0\% (3/25) & \cellcolor{BrickRed!11} 11.3\% (11/97)\\
\hline


==> tables/cmp_table_gdpr_preticked.tex <==
                        Quantcast & \cellcolor{BrickRed!37} 37.8\% (62/164) & \cellcolor{BrickRed!55} 55.0\% (33/60) & \cellcolor{BrickRed!32} 32.4\% (11/34) & \cellcolor{BrickRed!20} 20.0\% (6/30) & \cellcolor{BrickRed!60} 60.0\% (3/5) & \cellcolor{BrickRed!33} 33.3\% (4/12) & \cellcolor{BrickRed!21} 21.7\% (5/23)\\
                         OneTrust & \cellcolor{BrickRed!83} 83.3\% (40/48) & \cellcolor{BrickRed!93} 93.3\% (14/15) & \cellcolor{BrickRed!83} 83.3\% (5/6) & \cellcolor{BrickRed!100} 100.0\% (4/4) & \cellcolor{BrickRed!77} 77.8\% (7/9) & \cellcolor{BrickRed!66} 66.7\% (2/3) & \cellcolor{BrickRed!72} 72.7\% (8/11)\\
                      Sourcepoint & \cellcolor{BrickRed!64} 64.7\% (22/34) & \cellcolor{BrickRed!100} 100.0\% (21/21) & \cellcolor{BrickRed!0} 0.0\% (0/8) &                    -  &                    -  &                    -  & \cellcolor{BrickRed!20} 20.0\% (1/5)\\
                           Didomi & \cellcolor{BrickRed!39} 39.0\% (16/41) & \cellcolor{BrickRed!100} 100.0\% (1/1) & \cellcolor{BrickRed!24} 24.1\% (7/29) & \cellcolor{BrickRed!0} 0.0\% (0/1) & \cellcolor{BrickRed!100} 100.0\% (6/6) &                    -  & \cellcolor{BrickRed!50} 50.0\% (2/4)\\
                           OneTag & \cellcolor{BrickRed!100} 100.0\% (9/9) &                    -  &                    -  & \cellcolor{BrickRed!100} 100.0\% (9/9) &                    -  &                    -  &                    - \\
                   Commanders Act & \cellcolor{BrickRed!80} 80.0\% (8/10) &                    -  & \cellcolor{BrickRed!80} 80.0\% (8/10) &                    -  &                    -  &                    -  &                    - \\
                Conversant Europe & \cellcolor{BrickRed!100} 100.0\% (7/7) & \cellcolor{BrickRed!100} 100.0\% (1/1) &                    -  & \cellcolor{BrickRed!100} 100.0\% (3/3) &                    -  &                    -  & \cellcolor{BrickRed!100} 100.0\% (3/3)\\
                        Ensighten & \cellcolor{BrickRed!100} 100.0\% (7/7) & \cellcolor{BrickRed!100} 100.0\% (7/7) &                    -  &                    -  &                    -  &                    -  &                    - \\
                              SFR & \cellcolor{BrickRed!100} 100.0\% (4/4) &                    -  & \cellcolor{BrickRed!100} 100.0\% (4/4) &                    -  &                    -  &                    -  &                    - \\
                           Evidon & \cellcolor{BrickRed!25} 25.0\% (4/16) & \cellcolor{BrickRed!11} 11.1\% (1/9) &                    -  &                    -  &                    -  &                    -  & \cellcolor{BrickRed!42} 42.9\% (3/7)\\
                  Wikia. (FANDOM) & \cellcolor{BrickRed!100} 100.0\% (3/3) &                    -  &                    -  &                    -  &                    -  &                    -  & \cellcolor{BrickRed!100} 100.0\% (3/3)\\
                 Cookie Trust WG. & \cellcolor{BrickRed!60} 60.0\% (3/5) &                    -  & \cellcolor{BrickRed!100} 100.0\% (2/2) & \cellcolor{BrickRed!50} 50.0\% (1/2) & \cellcolor{BrickRed!0} 0.0\% (0/1) &                    -  &                    - \\
                    Axel Springer & \cellcolor{BrickRed!100} 100.0\% (3/3) &                    -  &                    -  & \cellcolor{BrickRed!100} 100.0\% (1/1) &                    -  &                    -  & \cellcolor{BrickRed!100} 100.0\% (2/2)\\
              Snigel Web Services & \cellcolor{BrickRed!75} 75.0\% (3/4) &                    -  & \cellcolor{BrickRed!100} 100.0\% (1/1) &                    -  &                    -  & \cellcolor{BrickRed!0} 0.0\% (0/1) & \cellcolor{BrickRed!100} 100.0\% (2/2)\\
                       Spil Games & \cellcolor{BrickRed!100} 100.0\% (3/3) & \cellcolor{BrickRed!100} 100.0\% (1/1) & \cellcolor{BrickRed!100} 100.0\% (1/1) & \cellcolor{BrickRed!100} 100.0\% (1/1) &                    -  &                    -  &                    - \\
                         TrustArc & \cellcolor{BrickRed!100} 100.0\% (3/3) &                    -  &                    -  &                    -  &                    -  &                    -  & \cellcolor{BrickRed!100} 100.0\% (3/3)\\
                  Livesport Media & \cellcolor{BrickRed!100} 100.0\% (3/3) &                    -  & \cellcolor{BrickRed!100} 100.0\% (1/1) & \cellcolor{BrickRed!100} 100.0\% (1/1) &                    -  &                    -  & \cellcolor{BrickRed!100} 100.0\% (1/1)\\
                  \textbf{others} & \cellcolor{BrickRed!23} 23.6\% (33/140) & \cellcolor{BrickRed!25} 25.0\% (7/28) & \cellcolor{BrickRed!40} 40.0\% (14/35) & \cellcolor{BrickRed!7} 7.4\% (4/54) & \cellcolor{BrickRed!100} 100.0\% (1/1) & \cellcolor{BrickRed!33} 33.3\% (1/3) & \cellcolor{BrickRed!31} 31.6\% (6/19)\\
\hline
           \setrow{\bfseries} all & \cellcolor{BrickRed!46} 46.5\% (236/508) & \cellcolor{BrickRed!60} 60.1\% (86/143) & \cellcolor{BrickRed!42} 42.1\% (56/133) & \cellcolor{BrickRed!28} 28.3\% (30/106) & \cellcolor{BrickRed!77} 77.3\% (17/22) & \cellcolor{BrickRed!36} 36.8\% (7/19) & \cellcolor{BrickRed!47} 47.1\% (40/85)\\
\hline


==> tables/cmp_table_tcf.tex <==
Quantcast & \cellcolor{gray!74} 74.3\% (133/179) & \cellcolor{gray!72} 72.1\% (129/179) \\\hline
OneTrust & \cellcolor{gray!52} 52.7\% (49/93) & \cellcolor{gray!48} 48.4\% (45/93) \\\hline
Sourcepoint & \cellcolor{gray!72} 72.7\% (32/44) & \cellcolor{gray!86} 86.4\% (38/44) \\\hline
Axel Springer & \cellcolor{gray!47} 47.6\% (20/42) & \cellcolor{gray!71} 71.4\% (30/42) \\\hline
Didomi & \cellcolor{gray!58} 58.5\% (24/41) & \cellcolor{gray!85} 85.4\% (35/41) \\\hline
Cookiebot & \cellcolor{gray!25} 25.0\% (7/28) & \cellcolor{gray!32} 32.1\% (9/28) \\\hline
Evidon & \cellcolor{gray!36} 36.4\% (8/22) & \cellcolor{gray!22} 22.7\% (5/22) \\\hline
iubenda & \cellcolor{gray!55} 55.0\% (11/20) & \cellcolor{gray!15} 15.0\% (3/20) \\\hline
Wirtualna Polska Media & \cellcolor{gray!0} 0.0\% (0/16) & \cellcolor{gray!0} 0.0\% (0/16) \\\hline
Clickio & \cellcolor{gray!60} 60.0\% (9/15) & \cellcolor{gray!100} 100.0\% (15/15) \\\hline
Livesport Media & \cellcolor{gray!0} 0.0\% (0/13) & \cellcolor{gray!0} 0.0\% (0/13) \\\hline
Oath & \cellcolor{gray!91} 91.7\% (11/12) & \cellcolor{gray!100} 100.0\% (12/12) \\\hline
Cookie Trust WG. & \cellcolor{gray!54} 54.5\% (6/11) & \cellcolor{gray!63} 63.6\% (7/11) \\\hline
Grupa Interia.pl & \cellcolor{gray!0} 0.0\% (0/10) & \cellcolor{gray!90} 90.0\% (9/10) \\\hline
Triboo Media & \cellcolor{gray!100} 100.0\% (10/10) & \cellcolor{gray!90} 90.0\% (9/10) \\\hline
Commanders Act & \cellcolor{gray!60} 60.0\% (6/10) & \cellcolor{gray!90} 90.0\% (9/10) \\\hline
OneTag & \cellcolor{gray!66} 66.7\% (6/9) & \cellcolor{gray!66} 66.7\% (6/9) \\\hline
Conversant Europe & \cellcolor{gray!75} 75.0\% (6/8) & \cellcolor{gray!87} 87.5\% (7/8) \\\hline
Ensighten & \cellcolor{gray!14} 14.3\% (1/7) & \cellcolor{gray!14} 14.3\% (1/7) \\\hline
SIRDATA & \cellcolor{gray!60} 60.0\% (3/5) & \cellcolor{gray!100} 100.0\% (5/5) \\\hline
Chandago & \cellcolor{gray!100} 100.0\% (5/5) & \cellcolor{gray!100} 100.0\% (5/5) \\\hline
\textbf{incorrect CMP ID} & \cellcolor{gray!31} 31.1\% (28/90) & \cellcolor{gray!66} 66.7\% (60/90) \\\hline
\textbf{others} & \cellcolor{gray!65} 65.3\% (49/75) & \cellcolor{gray!68} 68.0\% (51/75) \\\hline
\textbf{No consent string found} & \cellcolor{gray!30} 30.6\% (202/661) & \cellcolor{gray!44} 44.6\% (295/661) \\\hline
\setrow{\bfseries} all & \cellcolor{gray!43} 43.9\% (626/1426) & \cellcolor{gray!55} 55.0\% (785/1426) \\\hline


==> tables/country_preaction.tex <==
.uk & \cellcolor{BrickRed!11} 11.4\% (17/149) \\
.fr & \cellcolor{BrickRed!7} 7.2\% (10/139) \\
.pl & \cellcolor{BrickRed!17} 17.8\% (23/129) \\
.it & \cellcolor{BrickRed!9} 9.8\% (12/123) \\
.es & \cellcolor{BrickRed!7} 7.1\% (8/113) \\
.nl & \cellcolor{BrickRed!0} 0.0\% (0/65) \\
.gr & \cellcolor{BrickRed!3} 3.8\% (2/53) \\
.pt & \cellcolor{BrickRed!1} 1.9\% (1/52) \\
.de & \cellcolor{BrickRed!28} 28.6\% (16/56) \\
.ro & \cellcolor{BrickRed!2} 2.0\% (1/50) \\
.bg & \cellcolor{BrickRed!3} 3.8\% (1/26) \\
.fi & \cellcolor{BrickRed!10} 10.6\% (5/47) \\
.no & \cellcolor{BrickRed!2} 2.1\% (1/48) \\
.dk & \cellcolor{BrickRed!4} 4.9\% (2/41) \\
.be & \cellcolor{BrickRed!42} 42.1\% (16/38) \\
.at & \cellcolor{BrickRed!12} 12.1\% (4/33) \\
.ie & \cellcolor{BrickRed!12} 12.0\% (3/25) \\
.cz & \cellcolor{BrickRed!3} 3.6\% (1/28) \\
.ch & \cellcolor{BrickRed!0} 0.0\% (0/26) \\
.se & \cellcolor{BrickRed!9} 9.5\% (2/21) \\
.sk & \cellcolor{BrickRed!7} 7.1\% (1/14) \\
.hr & \cellcolor{BrickRed!0} 0.0\% (0/8) \\
.hu & \cellcolor{BrickRed!0} 0.0\% (0/6) \\
.lu & \cellcolor{BrickRed!0} 0.0\% (0/1) \\
.lt & \cellcolor{BrickRed!25} 25.0\% (1/4) \\
.lv & \cellcolor{BrickRed!0} 0.0\% (0/2) \\
.si & \cellcolor{BrickRed!0} 0.0\% (0/2) \\
.is & \cellcolor{BrickRed!0} 0.0\% (0/1) \\
.ee & \cellcolor{BrickRed!0} 0.0\% (0/1) \\
\hline
.com & \cellcolor{BrickRed!11} 11.3\% (11/97) \\
.org & \cellcolor{BrickRed!12} 12.5\% (2/16) \\
.eu & \cellcolor{BrickRed!8} 8.3\% (1/12) \\
\hline
\setrow{\bfseries} all & \cellcolor{BrickRed!9} 9.9\% (141/1426) \\
\hline


==> tables/websites_violation_nonrespect.tex <==
113 & reuters.com \\
151 & telegraph.co.uk \\
277 & sindonews.com \\
373 & softonic.com \\
562 & wowhead.com \\
841 & techtarget.com \\
1 085 & makeuseof.com \\
1 376 & bustle.com \\
1 420 & filehippo.com \\
1 618 & cdiscount.com \\
\hline


==> tables/websites_violation_nooption.tex <==
48 & msn.com \\
322 & healthline.com \\
345 & economist.com \\
545 & slate.com \\
706 & medicalnewstoday.com \\
849 & discogs.com \\
8 017 & ilmessaggero.it \\
8 842 & ticketmaster.co.uk \\
10 972 & tomshw.it \\
12 623 & ilgazzettino.it \\
\hline


==> tables/websites_violation_preaction.tex <==
48 & msn.com \\
373 & softonic.com \\
434 & merriam-webster.com \\
453 & britannica.com \\
545 & slate.com \\
551 & thesun.co.uk \\
706 & medicalnewstoday.com \\
821 & thetimes.co.uk \\
841 & techtarget.com \\
1 203 & vanityfair.com \\
\hline


==> tables/websites_violation_preticked.tex <==
58 & cnn.com \\
113 & reuters.com \\
119 & tinyurl.com \\
127 & bloomberg.com \\
133 & fandom.com \\
197 & w3schools.com \\
316 & mashable.com \\
373 & softonic.com \\
425 & wikia.com \\
434 & merriam-webster.com \\
\hline

